Studies of Systematic Uncertainties for Simons Observatory: Polarization Modulator Related Effects

The Simons Observatory (SO) will observe the temperature and polarization anisotropies of the cosmic microwave background (CMB) over a wide range of frequencies (27 to 270 GHz) and angular scales by using both small (0.5 m) and large (6 m) aperture telescopes. The SO small aperture telescopes will target degree angular scales where the primordial B-mode polarization signal is expected to peak. The incoming polarization signal of the small aperture telescopes will be modulated by a cryogenic, continuously-rotating half-wave plate (CRHWP) to mitigate systematic effects arising from slowly varying noise and detector pair-differencing. In this paper, we present an assessment of some systematic effects arising from using a CRHWP in the SO small aperture systems. We focus on systematic effects associated with structural properties of the HWP and effects arising when operating a HWP, including the amplitude of the HWP synchronous signal (HWPSS), and I -> P (intensity to polarization) leakage that arises from detector non-linearity in the presence of a large HWPSS. We demonstrate our ability to simulate the impact of the aforementioned systematic effects in the time domain. This important step will inform mitigation strategies and design decisions to ensure that SO will meet its science goals.

==> HWPmodel/HWPvsAngleAndNu_v0.tex <==
\label{sec:HWP_vs_angle_and_nu}

Sapphire is a positive uniaxial crystal. Assuming that it is cut with the optical axis parallel to the surfaces of the crystal in the x-y plane and can rotate by an angle $\chi$ with respect to the x-axis, the dielectric tensor of the crystal is
\begin{equation}
\epsilon=R(\chi)\begin{bmatrix}
n_e^2 &0 &0\\
0 &n_o^2 &0\\
0 &0 &n_o^2\\
\end{bmatrix}R(-\chi),
\end{equation}
where $R(\chi)$ is the usual $3\mathrm{x}3$ rotation matrix, and $n_o$ and $n_e$ are the ordinary and extraordinary indices of refraction, respectively~\cite{Essinger13}. If an electromagnetic wave of frequency $\nu$ is transmitted from a medium with index of refraction $n_1$ to a sapphire crystal with incidence angle $\theta$, the two components in which the linearly-polarized wave can be decomposed -- s- or TE and p- or TM waves -- are mixed inside the crystal to form the ordinary and extraordinary waves. The two components travel at different speeds through a uniaxial crystal. One component is refracted at an angle $\theta^{'}$ as given by Snell's law $n_1\sin\theta=n_o\sin\theta^{'}$ and travels with a speed $v_0=c/n_o$, while the other component is refracted at an angle $\theta^{"}$ as given by $n_1\sin\theta=n^{"}\sin\theta^{"}$ and travels with a speed $v^{"}=c/n^{"}$. The index of refraction $n^{"}$ is a function of $n_e$, the incidence angle $\theta$, and the rotation angle of the HWP $\chi$. It is given by~\cite{Essinger13}:
\begin{equation}
n^{"}=n_e\sqrt{1+(n_e^{-2}-n_o^{-2})n_1^2\sin^2\theta\cos^2\chi}.
\end{equation}

When traversing a layer of thickness $d$, the two components of the electromagnetic wave gain a phase difference of
\begin{equation}\label{eq:Gamma}
\Gamma=\frac{2\pi c}{\nu}d\,\left|\tilde{n}_o\cos\theta^{'}-\tilde{n}^{"}\cos\theta^{"}\right| \,\, ,
\end{equation}
where $\tilde{n}=n(1-i\tan\delta)^{1/2}$ is the complex index of refraction that takes into account the loss tangent $\tan(\delta)$ inside the material~\cite{Lamb1996}. The phase difference $\Gamma$ is effectively responsible for the rotation of the polarization direction of the electromagnetic wave transmitted through the HWP.

From Eq.~\ref{eq:Gamma}, it is clear that the effect induced by the HWP stack on the incoming wave depends on both the frequency of the wave and the incidence angle. In particular, at fixed $\theta$, the design of a single layer HWP can provide a $\Gamma=\pi$ phase difference for a single frequency $\nu_c$ only. For frequencies farther away from $\nu_c$, the retarder does not behave as an ideal HWP. The Mueller matrix of an ideal one-layer retarder with optical axis rotated by an angle $\alpha$, and that induces a phase difference of $\Gamma$ at $\theta=0$ is given by:
\begin{equation}\label{eq:Mij}
M_\mathrm{id}=\begin{bmatrix}
1 &0 &0 &0\\
0 &\cos^2(2\alpha)+\cos\Gamma \sin^2(2\alpha) &\cos(2\alpha)\sin(2\alpha)-\cos\Gamma\cos(2\alpha)\sin(2\alpha) &\sin(2\alpha)\sin\Gamma\\
0 &\cos(2\alpha)\sin(2\alpha)-\cos\Gamma\cos(2\alpha)\sin(2\alpha) &\cos\Gamma \cos^2(2\alpha)+\sin^2(2\alpha) &-\cos(2\alpha)\sin\Gamma\\
0 &-\sin(2\alpha)\sin\Gamma &\cos(2\alpha)\sin\Gamma &\cos\Gamma 
\end{bmatrix}.
\end{equation}

The Mueller matrix of an ideal three-layer retarder is given by inserting Eq.~\ref{eq:Mij} into Eq.~\ref{eq:Mstack2} as $M_2(\phi)$ with $\alpha=\phi$ and including the resulting matrix in Eq.~\ref{eq:Mstack_full} as $M_\mathrm{stack}$, with varying $\chi$. Figures~\ref{fig:Mij_one} and~\ref{fig:Mij_three} depict the elements $M_{i,j}$ for $i,j=1,2,3,4$ of a single-layer and three-layer Mueller matrix as a function of the frequency of the incoming wave and the incident angles $\theta=0^\circ,20^\circ$. The elements $M_{\mathrm{id},i,j}$ of the ideal matrix are shown as red dashed lines. It is clear that the elements $M_{\mathrm{id},i,j}$ resemble a HWP -- i.e. $\Gamma=\pi$ -- only at the central frequency $\nu_0\simeq 120$~GHz. The solid black line and the dotted-dashed cyan line correspond to the POLARBEAR2 HWP~\cite{Hill:2016jhd}, modeled through the TMM. The agreement with the ideal HWP is good for frequencies from 60~GHz to 180~GHz. Deviations from the ideal case $M_{\mathrm{id},i,j}$ are primarily due to differential properties of the Sapphire and absorption inside the material 
%(\textcolor{blue}{Are we sure of this?The wiggles could be due to the spectral trend of the sapphire refraction index. If you just plot the sapphire transmission you will get the same trend.}), 
which is modeled through the loss tangent. The visible wiggles at all frequencies are primarily induced by multiple reflections between the boundaries of the dielectric layers, which is mostly attenuated  with the AR coating. 
%(\textcolor{blue}{the AR does not attenuate the multiple reflections, they are still present. It attenuates the refraction index mismatch between the sapphire and the vacuum/air.})
The solid black line corresponds to $\theta=0^\circ$, while the dotted-dashed cyan line correspond to $\theta=20^\circ$. The difference between the two lines is barely visible, suggesting that the impact of the incidence angle on the behavior of the HWP is small but non-negligible.


\begin{figure}
\begin{center}
\includegraphics[width=0.7\textwidth]{plots/1layer_PB2_nu120_0_20deg}
\end{center}
\caption{Mueller matrix elements of a single-layer HWP as a function of the frequency $\nu$ of the incident wave. The design is that of the individual layers in the POLARBEAR (PB2) AHWP. The rotation angle is fixed and equal to $\chi=0$. The red lines correspond to an ideal retarder as defined in Eq.~\ref{eq:Mij}. The black line corresponds to the simulations based on the PB2 HWP design and computed with the TMM. The solid black line is for $\theta=0^\circ$, whereas the dotted-dashed cyan line is for $\theta=20^\circ$. %\textcolor{red}{Is the single layer like PB2 also? clarify.} 
%\textcolor{blue}{Leave out the zero components on this one and say in the caption which elements=0.}
}\label{fig:Mij_one}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.7\textwidth]{plots/3layer_PB2_nu120_0_20deg}
\end{center}
\caption{Mueller matrix elements of the three-layer POLARBEAR2 AHWP as a function of the frequency $\nu$ of the incident wave in the same style as Fig.~\ref{fig:Mij_one}. If compared with Fig.~\ref{fig:Mij_one}, the different behaviuor of the Mueller matrix elements with the incident frequency is clearly visible in the case of a three-layer AHWP. In particular, the number of non-zero components is reduced with respect to the single-layer HWP. The non-zero components also exhibit a more complicated dependence from the incident frequency than in the single-layer case. The main reason for these clearly visible differences posits in the extra-phase induced by the multi-layer stacking.}\label{fig:Mij_three}
\end{figure}


Figures~\ref{fig:Mij_diff_one} and~\ref{fig:Mij_diff_three} show the difference $M_{i,j}(\theta)-M_{i,j}(\theta=0)$ as a function of the rotation angle $\chi$ for a fixed frequency $\nu_0=120\,\mathrm{GHz}$, for a single-layer HWP and a three-layer AHWP, respectively. For the AHWP, the difference with respect to the $\theta=0$ case is always $<0.05$\footnote{We note that the AR coating plays a major role in keeping this difference low. In the absence of the AR coating, the difference can be a factor of a few higher.}. However, in Sec.~\ref{HWPSS_Intro}, we will see that this tiny difference can induce non-negligible effects.

\begin{figure}
\begin{center}
\includegraphics[width=0.7\textwidth]{plots/Mueller_elements_diff_1l}
\end{center}
\caption{Difference between the Mueller matrix elements for $\theta=10^\circ\,\mathrm{orange},\,20^\circ\,\mathrm{green}$ and $\theta=0^\circ$, of a single-layer HWP as a function of the rotation angle $\chi$. The frequency is fixed and equal to $\nu_0=120\,\mathrm{GHz}$. The figure shows that the difference between non-normal incidence and normal incidence is very small. However, as it is detailed in Sec.~\ref{HWPSS_Intro}, it is not negligible.}\label{fig:Mij_diff_one}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.7\textwidth]{plots/Mueller_elements_diff_3l_nu90}\\ \includegraphics[width=0.7\textwidth]{plots/Mueller_elements_diff_3l_nu150}
\end{center}
\caption{Difference between the Mueller matrix elements for a three-layer AHWP in the same style as Fig.~\ref{fig:Mij_diff_one}. The frequency is fixed and equal to $\nu_0=90\,\mathrm{GHz}$ (top panel) and $\nu_0=150\,\mathrm{GHz}$ (bottom panel).}\label{fig:Mij_diff_three}
\end{figure}



==> HWPmodel/Mueller_v0.tex <==
We make use of the generalized transfer matrix method (TMM) to model the optical action of sapphire HWPs. The TMM determines the relation between the transverse-magnetic (TM) and transverse-electric (TE) components of the incoming and outgoing radiation at the two boundaries of an optical element (or a stack of elements) using the boundary conditions. The TMM has several advantages. This method deals directly with the amplitudes of the fields at the interfaces of the two layers, and thus automatically takes multiple reflections between layers into account. The TMM is easy to generalize to multi-layer elements like broadband achromatic HWPs (AHWPs) with AR coatings. Finally, the TMM can be very easily applied to the more general case of arbitrary incidence angle and HWP rotation. Once the transfer matrix for the stack is computed, it is also possible to compute the corresponding Jones matrix and Mueller matrix\footnote{A public version of the code can be found at \url{https://github.com/tomessingerhileman/birefringent_transfer_matrix}, thanks to Tom Essinger-Hileman.} (see e.g.\cite{Abel50,Born99,Hecht87,Berreman72,Yeh79,Essinger13}).

For the SO HWP, we consider a three-layer AHWP built up from three individual HWPs with a two-layer AR coating (on each side) with thicknesses and indices of refraction matching the POLARBEAR2 AHWP design, which are reported in Tab.~\ref{tab:AHWP}~\cite{Hill:2016jhd}. The central HWP layer is rotated by $\phi=54^\circ$ with respect to the first layer, while the third layer is aligned with the first layer. Each birefringent layer of the AHWP is optimized for a central frequency of 120~GHz, and the stack can efficiently cover the two bands centered at 90~GHz and 150~GHz accordingly to the Pancharatnam
model\textcolor{red}{\cite{Pancharatnam55}}.


\begin{table}
\centering
\begin{tabular}{ |c|c|c|c| } 
  \hline
	 Layer & Thickness [mm] & Index of refraction & Loss tangent [$10^{-4}$] \Tstrut\\
  \hline
  AR top layer & 0.38 & 1.55 &   0.50 \Tstrut \\ 
  \hline
  AR bottom layer & 0.27 & 2.52 &  56.5 \\ 
  \hline
  \multirow{2}{*}{HWP layer} &\multirow{2}{*}{3.75}	&3.05 ($n_o$)	&2.0 ($\tan\delta_o$)\\
  &			&3.38 ($n_e$)	&1.0 ($\tan\delta_e$)\\
  \hline
\end{tabular}
\caption{\label{tab:AHWP}
Design of the AHWP used in this work. The design matches the POLARBEAR2 AHWP design~\cite{Hill:2016jhd}. The position of both the AR layers is symmetric with respect to the three HWP layers. $n_{o,e}$ are the indexes of refraction along the ordinary and extraordinary axes of the HWP. The loss tangent is in general a function of frequency~\cite{parshin_dielectric_1994,Hill:2016jhd,savini_achromatic_2006}. In this analysis, we have assumed a constant loss tangent with frequency along the two axes for the sake of simplicity~\cite{parshin_dielectric_1994}. 
}
\end{table}

The Mueller matrix for the single-layer HWP takes the generic form of Eq.~\ref{eq:Mueller}, which allows for leakage into off-diagonal terms\cite{Bryan:10}. In the case of the AHWP, Eq.~\ref{eq:Mueller} takes a different form to account for the fact that the AHWP is a stack of several layers rotated by a certain angle with respect to the first layer. Although we make use of the more rigorous approach of the TMM in this analysis, it is nevertheless instructive to work out the Mueller matrix of a generic HWP following an analytic approach in the case of normal incidence. 

In the case of a AHWP, each layer is represented by a Mueller matrix as in Eq.~\ref{eq:Mueller}, and the second layer $M_2(\phi)$ rotated by an angle $\phi$ with respect to the first layer can be modeled as:
\begin{equation}\label{eq:Mstack}
M_2 = R_M{(2\phi)}\cdot M_\mathrm{HWP} \cdot R_M(-2\phi),
\end{equation} 
where $R_M(2\phi)$ indicates the rotation matrix in Mueller formalism\cite{Collett93} by an angle $\phi$. In Eq.~\ref{eq:Mstack}, $\phi$ is constant in time and is defined by the design of the three-layer HWP, according to the Pancharatnam model. The global Mueller matrix for the three-layer stack can be finally computed as:
\begin{equation}\label{eq:Mstack2}
M_\mathrm{stack} = M_\mathrm{HWP}\cdot M_2(\phi) \cdot M_\mathrm{HWP}.
\end{equation} 

Eventually, the global rotation of the HWP stack can be modeled similarly:
\begin{equation}\label{eq:Mstack_full}
M_\mathrm{stack}(\chi) = R_M(2\chi)\cdot M_\mathrm{stack}(\chi=0) \cdot R_M(-2\chi),
\end{equation}
where $\chi$ is the global HWP rotation angle (see Eq.\ref{eq:demod_signal}). The latter changes with time as $\chi=2\pi f t$ and $f$ is the spinning frequency of the HWP ($f\approx 2\,\mathrm{Hz}$ for the SO CRHWP).






